LiDAR Snowfall Simulation for Robust 3D Object Detection

3D object detection is a central task for applications such as autonomous driving, in which the system needs to localize and classify surrounding traffic agents, even in the presence of adverse weather. In this paper, we address the problem of LiDAR-based 3D object detection under snowfall. Due to the difficulty of collecting and annotating training data in this setting, we propose a physically based method to simulate the effect of snowfall on real clear-weather LiDAR point clouds. Our method samples snow particles in 2D space for each LiDAR line and uses the induced geometry to modify the measurement for each LiDAR beam accordingly. Moreover, as snowfall often causes wetness on the ground, we also simulate ground wetness on LiDAR point clouds. We use our simulation to generate partially synthetic snowy LiDAR data and leverage these data for training 3D object detection models that are robust to snowfall. We conduct an extensive evaluation using several state-of-the-art 3D object detection methods and show that our simulation consistently yields significant performance gains on the real snowy STF dataset compared to clear-weather baselines and competing simulation approaches, while not sacrificing performance in clear weather. Our code is available at www.github.com/SysCV/LiDAR_snow_sim.

==> tables/wet_surface.tex <==
\begin{table}
\smaller
\centering
\begin{tabular}{ ll | rrrr  }
\multirow{2}{*}{\textbf{method}}& \textbf{data pre-}    & \multicolumn{4}{c}{\textbf{wet road and heavy snowfall} $\uparrow$}                   \\ 

                                & \textbf{processing}   & \notsotiny \textbf{0-80m} & \notsotiny 0-30m  & \notsotiny 30-50m & \notsotiny 50-80m \\

\hline \hline \noalign{\vskip 1mm} 

\multirow{4}{*}{PV-RCNN~\cite{PV-RCNN}} & \clear        & 25.95                     & 41.08             & 27.91             & \textbf{11.38}    \\ 
                                        & \wet          & 27.08                     & 44.86             & 26.92             & 11.01             \\
                                        & \snow         & \textbf{28.23}            & \textbf{44.87}    & \textbf{30.28}    & 10.10             \\
                                        & \both         & 27.50                     & 43.75             & 29.91             & 10.75             \\

\hline \noalign{\vskip 1mm} 

\multirow{4}{*}{VoxelRCNN~\cite{VRCNN}} & \clear        & 27.77                     & 48.31             & \textbf{27.90}    & 7.58              \\ 
                                        & \wet          & 26.60                     & 47.38             & 25.89             & 7.69              \\
                                        & \snow         & \textbf{28.33}            & \textbf{49.06}    & 27.01             & \textbf{8.25}     \\
                                        & \both         & & & & \\

\hline \noalign{\vskip 1mm} 

\multirow{4}{*}{CenterPoint~\cite{CP}}  & \clear        & 25.21                     & \textbf{41.74}    & 27.63             & 7.41              \\ 
                                        & \wet          & \textbf{25.84}            & 39.96             & \textbf{29.09}    & \textbf{10.60}    \\
                                        & \snow         & & & & \\
                                        & \both         & & & & \\

\hline \noalign{\vskip 1mm} 

\multirow{4}{*}{Part-A²~\cite{PartA2}}  & \clear        & 25.81                     & 45.66             & 25.06             & 9.60              \\ 
                                        & \wet          & 27.37                     & 46.57             & \textbf{30.26}    & 8.19              \\ 
                                        & \snow         & \textbf{27.87}            & \textbf{49.14}    & 24.56             & \textbf{10.75}    \\
                                        & \both         & & & & \\

\hline \noalign{\vskip 1mm} 

\multirow{4}{*}{PointRCNN~\cite{PRCNN}} & \clear        & 23.22                     & 41.73             & 21.24             & \textbf{6.91}     \\ 
                                        & \wet          & \textbf{24.63}            & \textbf{44.40}    & \textbf{24.67}    & 6.17              \\
                                        & \snow         & & & & \\
                                        & \both         & & & & \\

\hline \hline 

\end{tabular}
\caption{3D average precision (AP) of moderate cars on a test split with 135 samples containing \textbf{wet road and heavy snowfall}. Please refer to Table~\ref{table:snowfall} for the legend.}
\label{table:wet_just_harsh}
\end{table}



\begin{table}
\centering
\smaller
\begin{tabular}{ ll r | r }
\multirow{2}{*}{\textbf{method}}& \textbf{data pre-}    & \textbf{clear}            & \textbf{harsh}            \\ 
                                & \textbf{processing}   & \notsotiny \textbf{0-80m} & \notsotiny \textbf{0-80m} \\ 

\hline \noalign{\vskip 1mm} 

PV-RCNN~\cite{PV-RCNN}          & \clear            & \textbf{45.36}            & 25.95                     \\ 
PV-RCNN~\cite{PV-RCNN}          & \wet              & 44.81                     & \textbf{27.08}            \\ 

\noalign{\vskip 1mm} 

VoxelRCNN~\cite{VRCNN}          & \clear            & \textbf{45.19}            & \textbf{27.77}            \\ 
VoxelRCNN~\cite{VRCNN}          & \wet              & 44.15                     & 26.60                     \\ 

\noalign{\vskip 1mm} 

Part-A²~\cite{PartA2}           & \clear            & \textbf{42.81}            & 25.81                    \\ 
Part-A²~\cite{PartA2}           & \wet              & 41.92                     & \textbf{27.37}           \\ 

\noalign{\vskip 1mm} 

CenterPoint~\cite{CP}           & \clear            & \textbf{44.11}            & 25.21                    \\ 
CenterPoint~\cite{CP}           & \wet              & 43.85                     & \textbf{25.84}           \\ 

\noalign{\vskip 1mm} 

PointRCNN~\cite{PRCNN}          & \clear            & \textbf{41.79}            & 23.22                    \\ 
PointRCNN~\cite{PRCNN}          & \wet              & 41.70                     & \textbf{24.63}           \\

\noalign{\vskip 1mm} \hline \noalign{\vskip 1mm} 

\end{tabular}
\caption{3D average precision (AP) of moderate cars on a test split with 135 samples containing \textbf{wet road and heavy snowfall}. Please refer to Table~\ref{table:snowfall} for the legend.}
\label{table:wet}
\end{table}
